RITA: A Tool for Automated Requirements Classification and Specification from Online User Feedback

Context and motivation. Online user feedback is a valuable resource for requirements engineering, but its volume and noise make analysis difficult. Existing tools support individual feedback analysis tasks, but their capabilities are rarely integrated into end-to-end support. Problem. The lack of end-to-end integration limits the practical adoption of existing RE tools and makes it difficult to assess their real-world usefulness. Solution. To address this challenge, we present RITA, a tool that integrates lightweight open-source large language models into a unified workflow for feedback-driven RE. RITA supports automated request classification, non-functional requirement identification, and natural-language requirements specification generation from online feedback via a user-friendly interface, and integrates with Jira for seamless transfer of requirements specifications to development tools. Results and conclusions. RITA exploits previously evaluated LLM-based RE techniques to efficiently transform raw user feedback into requirements artefacts, helping bridge the gap between research and practice. A demonstration is available at: https://youtu.be/8meCLpwQWV8.

==> abstract.tex <==
\textbf{Context and motivation.}
Online user feedback provides a continuous and valuable source of information for requirements engineering (RE) in rapidly evolving software systems. While large language models (LLMs) have demonstrated strong potential to automate feedback analysis and support requirements specification, these capabilities are rarely integrated into cohesive, usable tools for practitioners.
\textbf{Problem.}
The absence of end-to-end tool support limits the practical adoption of LLM-based techniques for feedback-driven RE. Practitioners face difficulties in systematically analysing large volumes of noisy user feedback and transforming them into structured and actionable requirements artifacts in a reproducible and configurable manner.
\textbf{Solution.}
To address this challenge, we present RITA, a tool that integrates lightweight open-source LLMs into a unified workflow for feedback-driven RE. RITA supports automated user request classification, non-functional requirement identification, and natural-language requirements specification generation from online user feedback, allowing flexible model configuration and technique reuse. 
\textbf{Results and conclusions.} RITA operationalizes previously validated LLM-based RE techniques and enables efficient transformation of raw feedback into requirements artifacts. The tool bridges the gap between empirical research and practical application, supporting more systematic and scalable feedback-driven requirements development while highlighting opportunities for replication, comparison, and further evaluation. A demonstration of RITA is available at: https://www.youtube.com/watch?v=XXXXXXXXXXX

==> declaration.tex <==
The authors have no competing interests to declare that are relevant to the content of this article. ChatGPT-4~\cite{OpenAI2024ChatGPT4}  was used to improve the
readability, and the authors remain fully responsible for the final content.

==> related-work.tex <==
\section{Related Work}

Here we present related work  ...



==> tool-description-old1.tex <==
\section{Tool Description (3-5p)}

\subsection{User Flow and Screen Presentation (1-2p)}
This section describes how a user interacts with RITA through the user interface. The focus is on the end-to-end usage flow (screens, decisions, and outputs) over the implementation details.

\subsubsection{Screen Flow Overview}
RITA provides a guided workflow where the user configures a run, submits a job, reviews results, and optionally continues through requirements artefact generation. The typical interaction is:
\begin{enumerate}
    \item Upload a reviews file (TXT/CSV/Excel) and, for tabular files, select the relevant text column.
    \item Configure the run by selecting the classification type (User Request Type or NFR), the LLM model, and the prompt strategy.
    \item Submit the job and observe progress via the status indicator.
    \item Review outputs in the results table and download the results as a CSV file.
    \item Continue to generation steps for SRS and user stories, and optionally sync selected user stories to Jira.
\end{enumerate}

\subsubsection{Configuration Screen}
The interaction begins in the configuration panel, where the user defines the intent of the run and the inference setup. The user selects:
\begin{itemize}
    \item \textbf{Classification type:} User Request Type or NFR.
    \item \textbf{Model selection:} the LLM used for inference.
    \item \textbf{Prompt strategy:} the prompting template/approach applied for the selected type.
\end{itemize}
This configuration-first approach supports experimentation: the same dataset can be rerun with different models or strategies to compare outputs without changing the input file.

\subsubsection{File Upload and Input Preparation}
After configuring the run, the user uploads their dataset of reviews. RITA supports common formats such as CSV/Excel and plain text. For tabular files, the user chooses the column containing review text to ensure the system processes the intended input. For CSV file, user selects the column based on the 'comma' delimiter as the index. This step enables the tool to handle datasets from different sources while keeping the user workflow consistent.

\subsubsection{Job Execution and Progress Feedback}
Once the input and configuration are set, the user submits the job. The frontend transitions into an execution state and provides progress feedback (e.g., processed reviews out of total reviews). This helps the user understand how the run is progressing, especially for larger datasets or slower model configurations. If an incorrect configuration was chosen, the user may cancel the job and restart with updated settings.

\subsubsection{Results Presentation and Export}
When processing completes, the results view presents the outputs in a structured table. The user can inspect classifications per review entry and download the final output as a CSV file for reporting, manual validation, or downstream analysis. The export step is intentionally integrated into the workflow to support reuse of results outside the application.

\subsubsection{Generation and Integration Flow}
Beyond classification, RITA supports downstream requirements engineering artefact generation from the classified feedback, using the same interaction pattern (configure $\rightarrow$ submit $\rightarrow$ view output):
\begin{itemize}
    \item Generate Software Requirements Specification (SRS).
    \item Generate user stories.
\end{itemize}
In addition, RITA provides an integration step for project tracking:
\begin{itemize}
    \item Sync \textit{selected} user stories to Jira as issues (optional, requires user selection and Jira configuration).
\end{itemize}
This design allows users to stop after classification when they only need structured labels and exports, or to continue through a full pipeline from raw reviews to formalised artefacts and task tracking.




\subsection{Overview of the RITA Architecture (2-3p)}

\FloatBarrier

To better understand the structure and behaviour of the Requirements Engineering Tool (RITA), the following UML diagrams are presented:
\begin{itemize}
    \item Component Diagram -- Illustrates the high-level modules (UI, API, Worker, database, and external services) and their interactions.
    \item Use Case Diagram -- Defines key actors and how they interact with RITA’s features (classification, generation, and Jira sync).
    \item Deployment Diagram -- Shows how the system components are deployed and how they communicate at runtime.
    \item Sequence Diagram -- Demonstrates the end-to-end flow for a typical classification job, from file upload to results.
\end{itemize}
 \FloatBarrier  

\subsubsection{Component Diagram}

The component diagram shows RITA as a simple service-oriented setup where a frontend UI communicates with an API service, while a worker processes jobs asynchronously. The key components are:
\begin{itemize}
    \item React UI: Collects user inputs (classification type, model, strategy) and uploads review files.
    \item API Service (FastAPI): Exposes HTTP endpoints to submit jobs, monitor progress, cancel execution, and trigger generation flows.
    \item Worker Service: Runs independently, polling queued jobs and performing the classification or generation tasks.
    \item Shared Database (SQLite): Acts as a lightweight decoupling mechanism by storing job state, input reviews, and results.
    \item Configuration Manager: Loads prompt templates, model mappings, and strategy options for consistent behavior across API and Worker.
    \item Client Modules: LLM client for Ollama calls, and Jira client for creating issues in Jira Cloud.
\end{itemize}
\FloatBarrier

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_component_diagram.png}
    \caption{Component Diagram of RITA}
    \label{fig:rita_component_diagram}
\end{figure}
\FloatBarrier


\subsubsection{Use Case Diagram}

\FloatBarrier
The use case diagram outlines how a user interacts with RITA for requirements engineering tasks:
\begin{itemize}
    \item User Request Type Classification: Classifies reviews into Functional Requirement Statements (e.g., feature request / bug report / other).
    \item NFR Classification: Classifies reviews into non-functional categories (e.g., usability, performance, reliability).
    \item Upload Reviews: Accepts input as TXT/CSV/Excel and extracts the target review column.
    \item Configure Model and Strategy: Selects an LLM option and a prompt strategy for the chosen classification mode.
    \item Submit Job and Monitor Progress: Creates a background job and tracks completion counts.
    \item Cancel Job: Stops processing by removing queued/running jobs.
    \item Download Results: Exports the classification output after completion.
    \item Generate SRS: Produces an SRS document from review text using a selected model/strategy.
    \item Generate User Stories: Produces user stories from classified feedback or SRS content.
    \item Sync to Jira: Sends selected user stories as Jira issues in a target project.
\end{itemize}
\FloatBarrier

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_use_case_diagram.png}
    \caption{Use Case Diagram of RITA}
    \label{fig:rita_use_case_diagram}
\end{figure}
\FloatBarrier

\subsubsection{Deployment Diagram}

\FloatBarrier
The deployment diagram describes how RITA executes in a real-world environment:
\begin{itemize}
    \item Client Device: A web browser runs the frontend UI and communicates with the API service over HTTP.
    \item API Host/Container: FastAPI serves the UI entry page and exposes REST endpoints on port 8002.
    \item Worker Host/Container: A separate worker process runs independently and polls the shared database.
    \item Shared State: A local SQLite database file is shared between the API and Worker to store job state and results.
    \item External Services: Ollama provides local inference over HTTP, while Jira Cloud is accessed over the internet via REST API.
\end{itemize}
\FloatBarrier

\FloatBarrier
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_deployment_diagram.png}
    \caption{Deployment Diagram of RITA}
    \label{fig:rita_deployment_diagram}
\end{figure}

\subsubsection{Sequence Diagram}
The sequence diagram represents the workflow for a typical classification job:
\begin{itemize}
    \item The user selects either User Request Classification (FRS) or NFR Classification, chooses an LLM and prompt strategy, and uploads a review file.
    \item The React UI calls the API to submit a job; the API stores the job in SQLite with status \texttt{QUEUED}.
    \item The worker polls the database, detects queued jobs, marks them \texttt{RUNNING}, and loads prompts/configuration.
    \item For each review, the worker calls Ollama via the LLM client, receives a label/output, and updates completion counters/results.
    \item Once all reviews are processed, the worker marks the job \texttt{COMPLETED}.
    \item The UI calls the API \texttt{/check\_status} to fetch progress and display results when complete. To be precise, the frontend UI uses a 500ms (0.5s) interval for classification polling and a 1000ms (1s) interval for Jira polling.
    \item Optional flows extend the same pattern for SRS generation, user story generation, and Jira synchronization.
\end{itemize}
\FloatBarrier

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_sequence_diagram1.png}
    \caption{Sequence Diagram of RITA (Classification Workflow)}
    \label{fig:rita_sequence_diagram1}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_sequence_diagram2.png}
    \caption{Sequence Diagram of RITA (Generation Workflow)}
    \label{fig:rita_sequence_diagram2}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_sequence_diagram3.png}
    \caption{Sequence Diagram of RITA (JIRA Sync Workflow)}
    \label{fig:rita_sequence_diagram3}
\end{figure}
\FloatBarrier



\subsection{Use Case Realisation}
\label{sec:use-case-realisation}

Description and figures presenting sequence / workflow diagram to realize use cases. \\

This section details how the RITA architecture operationalises its core use cases by tracing execution flow through the system’s decoupled components.

\subsubsection{UC-1: Review Classification and Artefact Generation}
\label{sec:uc1-classification-generation}

RITA adopts a clean-slate, single-job execution model. To ensure deterministic execution and prevent resource contention during compute-intensive LLM inference, the system maintains exactly one active job state. Every new submission triggers a global purge of the database, clearing previous records before initialising a new entry.

Jobs are handled via a FIFO (First-In-First-Out) strategy, following a linear state machine: \\
\texttt{QUEUED} $\rightarrow$ \texttt{RUNNING} $\rightarrow$ \texttt{COMPLETED}.
The worker, operating as a persistent background process, atomically transitions a job to \texttt{RUNNING} to ``lock'' the task before execution begins.

\paragraph{Classification (FR/NFR).}
The worker processes reviews sequentially. After each LLM inference call, the result is appended to the evolving state and immediately committed to the database. This granular persistence enables real-time progress telemetry and partial result visibility in the frontend.

\paragraph{Generation (SRS/User Stories).}
These tasks are treated as single-shot synchronous operations. Progress updates remain binary; the state jumps from 0\% to 100\% only upon the successful commit of the fully generated Markdown string.

\paragraph{Cancellation.}
Upon a cancellation request, the API deletes the job record. The worker, which performs an existence check during execution, detects the missing record and terminates gracefully, discarding in-memory volatile state.

\paragraph{Fault tolerance.}
RITA implements \texttt{FAILED} state and the errors within individual LLM calls are captured as error-string payloads within the results. This prevents a single failed inference from aborting a multi-review batch.

\subsubsection{UC-2: Jira Synchronisation}
\label{sec:uc2-jira-sync}

Jira integration is realised as a sequential background task. The worker iterates through the generated user stories, submitting them to the Jira Cloud API. To comply with standard API rate-limiting and ensure transmission reliability, a fixed 500\,ms delay is enforced between requests. The system maintains an audit trail by recording the resulting Jira issue keys or HTTP error messages directly within the job's result field.



\subsection{Implementation}

description of the technologies; and mapping to components 

This section describes the key implementation decisions underlying RITA, with emphasis on state management, execution semantics, and infrastructure trade-offs made during iterative prototyping.

\subsubsection{State Management and Persistence}

RITA employs a local SQLite database as a shared blackboard for coordinating interactions between the API layer and the background worker. The database is stored within the container’s internal filesystem and acts as the single source of truth for job configuration, execution state, and intermediate results.

Persistence is intentionally ephemeral. While the database survives process crashes or container restarts, it is reset during deployment cycles (e.g., \texttt{docker-compose down}) as no external host volumes are mounted. This design choice ensures that each experimental run begins from a known-empty state, preventing stale artefacts or schema drift from influencing subsequent evaluations.

To further enforce state clarity, the API performs a global purge of the jobs table prior to each new submission. This ``clean-slate'' policy guarantees that at most one active job exists at any given time, simplifying coordination logic and avoiding ambiguity in frontend progress reporting.

\subsubsection{Execution Model and Concurrency}

RITA is deployed as a unified single-container application. Both the FastAPI server and the background worker process are launched via a shared container entrypoint, allowing them to operate within the same filesystem and execution context.

Task execution is strictly sequential. The worker polls the database at fixed intervals and processes one job at a time, atomically transitioning its status to \texttt{RUNNING} before beginning execution. All classification, generation, and synchronisation tasks are performed synchronously, without batching or parallelism.

This execution model prioritises determinism and architectural simplicity over throughput. Given that local LLM inference constitutes the primary performance bottleneck, introducing concurrency was deemed unlikely to yield proportional gains while significantly increasing system complexity.

\subsubsection{Frontend and Infrastructure}

The frontend is implemented as a single static HTML file using React via CDN, with JSX transpiled in-browser through Babel. This build-less approach avoids reliance on external toolchains (e.g., Node.js, bundlers) and allows the entire system to be distributed as a lightweight Python-based artefact.

The frontend remains stateless across reloads and derives its runtime state exclusively from periodic API polling. Progress indicators, result tables, and generated artefacts are rendered solely based on the backend-reported job state.

\subsubsection{Inference and External Integration}

All LLM inference is delegated to a locally hosted Ollama instance accessed via a host-gateway bridge. This design ensures full data locality, eliminates usage-based costs, and enables reproducible experimentation under controlled model configurations.

Jira integration is implemented as an optional background task. Credentials are passed as part of the job payload and stored transiently within the database for the duration of the synchronisation process. These credentials persist in the database until the next "clean-slate" purge or a manual database reset, such as cancellation, or the initiation of a new task, limiting their exposure within the system.



==> tool-description-old2.tex <==
\section{Tool Description (3-5p)}

\subsection{User Flow and Screen Presentation}
This section outlines how users interact with RITA’s interface, focusing on the end-to-end usage flow—such as screens, user decisions, and outputs—rather than implementation details.


%\FloatBarrier

\subsubsection{Screen Flow Overview}
RITA provides a guided workflow that allows the user to configure the classification, initiate the classification process, review the results, and optionally proceed to generate requirements artefacts. The typical user interaction is as follows:
\begin{enumerate}
    \item Upload a file containing reviews (e.g., TXT, CSV, or Excel) and select the relevant column for text data if applicable.
    \item Configure the classification by choosing the classification type (such as User Request Type or Non-Functional Requirement), selecting the LLM model, and applying the appropriate prompt strategy.
    \item Initiate the classification process and monitor its progress via a status indicator.
    \item Review the results presented in a structured table and download the output as a CSV file.
    \item Optionally, proceed to generate Software Requirements Specifications (SRS) and user stories, and export selected user stories to Jira if needed.
\end{enumerate}

%\FloatBarrier

\subsubsection{Configuration Screen}
The interaction begins in the configuration panel, where the user defines the intent of the run and sets up the inference parameters. In this step, the user selects the classification type (either User Request Type or Non-Functional Requirement), chooses the LLM used for inference, and applies the appropriate prompt strategy. This configuration-first approach allows users to experiment with different models and strategies on the same dataset without modifying the input file.

%\FloatBarrier
\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/screenshots/File upload.png} % Replace with your actual image file
    \caption{Screenshot of Configuration screen for selecting classification type and model}
    \label{fig:config}
\end{figure}


\subsubsection{File Upload and Input Preparation}
After configuring the run, the user uploads their dataset of reviews. RITA supports common formats such as CSV, Excel, and plain text. For tabular files, the user selects the column containing the review text to ensure that the system processes the intended input. This step enables the tool to handle datasets from different sources while maintaining a consistent user workflow.

\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/screenshots/Process Reviews.png} % Replace with your actual image file
    \caption{Screenshot of  Requirement Classifier after User Attributes Selection}
    \label{fig:upload}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/screenshots/Processing Reviews.png} % Replace with your actual image file
    \caption{Screenshot of Processing of Classification Job}
    \label{fig:processing}
\end{figure}

\FloatBarrier

\subsubsection{Classification and Progress Feedback}
Once the input and configuration are finalized, the user initiates the user initiates the classification process. During this phase, the frontend transitions into an execution state and provides real-time progress feedback, such as the number of reviews processed out of the total. This helps the user understand the progress of the run, particularly for larger datasets or more complex model configurations. If an incorrect configuration is chosen, the user can cancel the job and restart it with updated settings.


\subsubsection{Results Presentation and Export}
Upon completion of the processing, the results are presented in a structured table format. Users can review the classification outputs for each review entry and download the final results as a CSV file. This export capability allows for easy reporting, manual validation, or further analysis outside the application.

\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/screenshots/Processed Reviews.png} % Replace with your actual image file
    \caption{Screenshot of Completion of Classification Progress}
    \label{fig:results}
\end{figure}


\subsubsection{Generation and Integration Flow}
Beyond classification, RITA supports the generation of requirements artefacts from the classified feedback. Using the same configuration and submission pattern (configure, execute, and review output), users can generate Software Requirements Specifications (SRS) and user stories. Additionally, RITA includes an integration step that allows users to export selected user stories as Jira issues, if desired. This design enables users to either stop after classification for simple labeling and export or proceed through a full pipeline from raw reviews to formalized artefacts and project tracking.

\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/screenshots/Generating SRS.png} % Replace with your actual image file
    \caption{Screenshot of SRS/User Story Processing Stage}
    \label{fig:srs}
\end{figure}


\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/screenshots/Generated User Stories.png} % Replace with your actual image file
    \caption{Screenshot of Generated User Stories}
    \label{fig:stories}
\end{figure}

\FloatBarrier

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/screenshots/JIRA config.png} % Replace with your actual image file
    \caption{Screenshot of Jira configuration}
    \label{fig:jira}
\end{figure}

\FloatBarrier




\newpage
\subsection{Overview of the RITA Architecture}

\FloatBarrier

This section provides a high-level overview of the RITA architecture. We include several UML diagrams to illustrate the system’s structure and interactions. These diagrams include a component diagram showing the main modules and how they interact, a use case diagram that details user interactions, a deployment diagram that explains how components are arranged in the environment, and a sequence diagram showing the typical workflow.

 \FloatBarrier  

\subsubsection{Component Diagram}
The RITA architecture consists of several core modules designed to separate user interaction from heavy data processing. 

The \textbf{React UI} provides a graphical interface where users manage their projects. It receives user inputs and files as \textit{input} and produces structured requests for the backend as \textit{output}. The \textbf{FastAPI service} functions as the central backend of RITA. It receives user requests from the interface, coordinates the processing tasks, and sends the finalized results back to the UI for display. 

To handle intensive tasks without freezing the interface, a \textbf{Worker Service} manages the background workload. It takes raw feedback data as \textit{input} and produces classified requirements as \textit{output}. These results are stored in a \textbf{Shared Database}, which acts as a storage hub that receives processed data from the worker and provides status information to the API. Finally, \textbf{LLM Clients} are required to bridge RITA with artificial intelligence models; they take text descriptions as \textit{input} and return predicted categories or generated requirements as \textit{output}, enabling the tool’s automated analysis capabilities.

\FloatBarrier

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_component_diagram.png}
    \caption{Component Diagram of RITA}
    \label{fig:rita_component_diagram}
\end{figure}
\FloatBarrier


\subsubsection{Use Case Diagram}

\FloatBarrier
%The use case diagram highlights the ways a user interacts with RITA to perform various requirements engineering tasks. Users can classify reviews into user-request types, such as features or bugs, or as non-functional attributes like usability and performance. They can upload reviews in various formats, configure the model and prompt strategy, and then submit a job to start the classification process. Throughout the process, they can monitor progress, cancel jobs if needed, and download the results once the classification is complete. Additionally, RITA allows users to generate Software Requirements Specifications and user stories from the classified data. They can also sync selected user stories to Jira, making it easy to integrate with existing project tracking tools.

The use case diagram illustrates RITA’s functionality from the user’s perspective, focusing on the value-add features rather than internal system processes. Inside the system boundary, the user can perform the following primary actions:
\begin{itemize}
    \item \textbf{Classify feedback:} Categorize reviews into User Request Type or Non-Functional Requirement.
    \item \textbf{Generate SRS:} Create formal software requirements specifications from analyzed data.
    \item \textbf{View and Download results:} Inspect the system's findings and export them for external use.
    \item \textbf{Export user stories to Jira:} Transfer generated requirements directly into project management workflows.
\end{itemize}

\FloatBarrier

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_use_case_diagram.png}
    \caption{Use Case Diagram of RITA}
    \label{fig:rita_use_case_diagram}
\end{figure}
\FloatBarrier

\subsubsection{Deployment Diagram}

\FloatBarrier


RITA is deployed using a distributed approach to ensure stability and accessibility. The user accesses the system via a web browser on a client device, which connects to the backend server over a standard network connection. The backend API and the background worker are hosted within containers to maintain a consistent environment. These components share a local database file to stay synchronized. For its intelligence features, the system communicates with an Ollama instance for local model execution and connects to the Jira Cloud service via the internet for task integration.

\FloatBarrier

\FloatBarrier
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_deployment_diagram.png}
    \caption{Deployment Diagram of RITA}
    \label{fig:rita_deployment_diagram}
\end{figure}

%\subsubsection{Sequence Diagram}
%This section illustrates the realization of the classification use case through the interaction of system components. When a user initiates a classification, the React UI sends the selected configuration and dataset to the API Service. The API Service then authenticates the request and initializes a job record in the Shared Database. The Worker Service, identifying the new entry, retrieves the raw reviews, processes them via the LLM Client, and stores the resulting classifications back into the database. Finally, the UI retrieves these processed results via the API to display them to the user. This collaborative flow ensures that heavy computation is decoupled from the user interface, maintaining system responsiveness.




\FloatBarrier

\subsection{Sequence Diagram and Use Case Realisation}
\label{sec:use-case-realisation}

\FloatBarrier

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/rita_sequence_diagram.png}
    \caption{Sequence Diagram of RITA (Classification Workflow)}
    \label{fig:rita_sequence_diagram}
\end{figure}

Figure~\ref{fig:rita_sequence_diagram} presents a unified sequence diagram illustrating a representative end-to-end interaction in RITA. The diagram focuses on the core classification scenario and highlights how system components collaborate to transform raw app reviews into structured requirements. Consistent with the principles outlined in \textit{Reference Architecture and Use Case for App Review Mining}, the diagram abstracts away low-level execution details and emphasises user-oriented system behaviour.

\subsubsection{UC-1: Review Classification and Artefact Generation}

The primary use case supported by RITA is the transformation of raw app reviews into structured requirements artefacts. The process begins when the user uploads a dataset of reviews and selects a classification type, language model, and prompt strategy through the user interface. These inputs are forwarded to the API service, which coordinates execution with the worker component.

The worker performs review-level analysis by invoking the language model to classify each review. The resulting classifications are progressively made available to the user, enabling visibility into processing progress and intermediate outputs. The outcome of this phase is a structured representation of the input reviews, categorised as User Request Type or Non-Functional Requirement.

Following classification, the same interaction pattern supports artefact generation. The classified outputs are used as contextual input to generate higher-level artefacts such as a Software Requirements Specification (SRS) or a set of user stories. These steps produce complete artefacts that users can review and export.

\subsubsection{UC-2: Integration with Project Management Tools}

RITA further supports integrating generated user stories into existing development workflows. After reviewing the generated output, the user can select one or more user stories and synchronise them with an external project management system such as Jira Cloud. Once synchronised, the user stories become available directly within Jira for planning and implementation activities.

\subsubsection{Interaction Summary}

Together, the unified sequence diagram and accompanying narrative describe how user actions propagate through the user interface, backend services, worker logic, and external integrations. By focusing on functional interactions rather than internal execution mechanics, this section demonstrates how RITA realises its core use cases of classification, requirements generation, and optional workflow integration.



\subsection{Implementation}

RITA is a lightweight, Docker-containerised system consisting of a React frontend, a FastAPI backend, a background worker, and local integrations with external services such as Jira. The frontend is implemented using React and provides a simple, stateless interface for uploading review datasets, configuring classification options, and viewing results. The backend API, built with FastAPI, coordinates user requests and mediates communication between the interface, the worker, and external services. A background worker component performs computationally intensive tasks such as review classification, requirements generation, and optional Jira synchronisation. A local SQLite database is used for transient state management and result persistence during execution.LLM inference is handled via a locally hosted Ollama service to ensure data locality and reproducibility, while Jira Cloud integration enables optional export of generated user stories into existing project management workflows. We also utilise GitHub Actions as part of our CI/CD validation process.This technology stack was selected to prioritise simplicity, transparency, and reproducible experimentation over deployment scalability.

RITA is a lightweight, Docker-containerised system consisting of a React frontend, a FastAPI backend, a background worker, and local integrations with external services such as Jira. The frontend is implemented in React and provides a simple stateless interface for uploading review datasets, configuring classification options and viewing results. The backend API is implemented using FastAPI and coordinates user requests while mediating communication between the frontend, the background worker and external services.A background worker performs computationally intensive tasks such as review classification, requirements generation and optional Jira synchronisation. A local SQLite database is used for transient state management and result persistence during execution.LLM inference is handled via a locally hosted Ollama service to ensure data locality and reproducibility while Jira Cloud integration enables optional export of generated user stories into existing project management workflows. GitHub Actions is used as part of the CI/CD validation process.This technology stack was selected to prioritise simplicity, transparency and reproducible experimentation over deployment scalability.





==> use-case.tex <==
\section{Motivation and Use Case: Requirements Classification and Specification (0.5-0.75p)}

requirements, functionalities, description motivating the tool comes here

Motivate the need for the tool, Describe the goals, requirements, intended users, and context of the use of the tool.


